Training microrobots to swim by a large language model

Machine learning and artificial intelligence have recently represented a popular paradigm for designing and optimizing robotic systems across various scales. Recent studies have showcased the innovative application of large language models (LLMs) in industrial control [1] and in directing legged walking robots [2]. In this study, we utilize an LLM, GPT-4, to train two prototypical microrobots for swimming in viscous fluids. Adopting a few-shot learning approach, we develop a minimal, unified prompt composed of only five sentences. The same concise prompt successfully guides two distinct articulated microrobots -- the three-link swimmer and the three-sphere swimmer -- in mastering their signature strokes. These strokes, initially conceptualized by physicists, are now effectively interpreted and applied by the LLM, enabling the microrobots to circumvent the physical constraints inherent to micro-locomotion. Remarkably, our LLM-based decision-making strategy substantially surpasses a traditional reinforcement learning method in terms of training speed. We discuss the nuanced aspects of prompt design, particularly emphasizing the reduction of monetary expenses of using GPT-4.

==> acknowledgement.tex <==
%We thank the helpful discussions with XXX. 
Z.X. is supported by the research scholarship from the National University of Singapore and the China Scholarship Council. L.Z. acknowledges the partial support from
the A*Star AME-YIRG grant (A2084c0175). Some computation of the work was performed on resources of the National Supercomputing Centre, Singapore (https://www.nscc.sg).
%as well as the supercomputer Fugaku provided by RIKEN through the HPCI System Research Project (Project ID: hp230185).

%Z.X. is supported by the research scholarship from the National University of Singapore and the China Scholarship Council. L.Z. acknowledges the Singapore Ministry of Education Academic Research Fund Tier 2 (MOE-T2EP50221-0012 \& MOE-T2EP50122-0015) and Tier 1 (A-8000197-01-00) grants, and the A*Star AME-YIRG grant (A2084c0175). Some computation of the work was performed on resources of the National Supercomputing Centre, Singapore (https://www.nscc.sg), as well as the supercomputer Fugaku provided by RIKEN through the HPCI System Research Project (Project ID: hp230185).


